Analysis of Microstate Organization During Emotional Events

Understanding the dynamics of emotional experience is an old problem. However, a clear understanding of the mechanism of emotional experience is still far away. In the presented work, we tried to address this problem using a well-established method called microstate analysis using multichannel electroencephalography (EEG). We recorded the brain activity of spontaneous emotional experiences while participants were watching multimedia emotional stimuli. The time duration where the participants spontaneously felt an emotion, we termed it an emotional event. Microstate segmentation is performed for all emotional events to calculate the set of microstates (MS). Followed by a comparison of calculated statistical parameters and transition probabilities for the emotional and non-emotional conditions. We found a set of MS (four MS) for emotional and non-emotional conditions that differ from each other. We observed that MS1 has a higher value of occurrence, duration and coverage for emotional conditions. In addition, the transition to MS1 for the emotional condition was higher. On the other hand, for non-emotion (or neutral) condition, transition to MS3 was higher. A set of MS related to neutral condition was source localized to brain regions involved in higher-level sensory feature processing. On the other hand, for emotional conditions, MS1 \& MS2 are localized to sensory feature processing regions, and MS3 \& MS4 are additionally localized to regions related to socio-emotional processing. Our results hint toward the constructionist mechanism, which has an asymmetric contribution from bottom-up and top-down processing during an emotional experience.

==> CodeInformation.tex <==
/media/sudhakar/4080C90A80C9077E/698GBDrive/ForMSAAnalysis/CalcEmtProb.py
/media/sudhakar/4080C90A80C9077E/698GBDrive/ForMSAAnalysis/MicrostateSourceLocalization.py
/mnt/8068a573-f543-43aa-8252-d1bf146726fa/ForMSAAnalysis/topoplotDiff.py
/media/sudhakar/4080C90A80C9077E/698GBDrive/ForMSAAnalysis/MicroStateComp.R
/home/zuddler/ForMSAAnalysis/MicrostateSourceLocalization.py

==> Old_Table.tex <==
\begin{table}[H]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|cccccccc}
 & \textbf{Group-01} & \textbf{Group-02} & \textbf{Group-03} & \textbf{Group-04} & \textbf{Group-05} & \textbf{Group-06} & \textbf{Group-07} & \textbf{Group-08} \\ \hline
\textbf{Group-01} & 0    & 0.91 & 0.66 & 0.69 & 0.7  & 0.72 & 0.79 & 0.76 \\
\textbf{Group-02} & 0.91 & 0    & 0.52 & 0.48 & 0.75 & 0.8  & 0.78 & 0.74 \\
\textbf{Group-03} & 0.66 & 0.52 & 0    & 0.12 & 0.62 & 0.85 & 0.79 & 0.75 \\
\textbf{Group-04} & 0.69 & 0.48 & 0.12 & 0    & 0.62 & 0.83 & 0.79 & 0.75 \\
\textbf{Group-05} & 0.7  & 0.75 & 0.62 & 0.62 & 0    & 0.64 & 0.66 & 0.79 \\
\textbf{Group-06} & 0.72 & 0.8  & 0.85 & 0.83 & 0.64 & 0    & 0.19 & 0.53 \\
\textbf{Group-07} & 0.79 & 0.78 & 0.79 & 0.79 & 0.66 & 0.19 & 0    & 0.41 \\
\textbf{Group-08} & 0.76 & 0.74 & 0.75 & 0.75 & 0.79 & 0.53 & 0.41 & 0  \\ \hline
\end{tabular}%
}
\caption{\textbf{Distance between prototypes for upper beta band:} The cell values in the table shows the mean distance between emotion groups' prototypes. The mean and median value calculated over all the distances mentioned in the table is 0.67 \& 0.73, respectively.
% sftp://silp150@172.17.25.150/mnt/8068a573-f543-43aa-8252-d1bf146726fa/ForMSAAnalysis/topoplotDiff.py
}
\label{tab:protodist}
\end{table}

\begin{table}[H]
\begin{tabular}{cccccccccc}
& \textbf{Neutral} & \textbf{Group-01} & \textbf{Group-02} & \textbf{Group-03} & \textbf{Group-04} & \textbf{Group-05} & \textbf{Group-06} & \textbf{Group-07} & \textbf{Group-08} \\
\textbf{Baseline} & 1.56(NS) & 1.56  & 1.48  & 1.56  & 1.55  & 1.31  & 1.04  & 1.03  & 1.25  \\
\textbf{Neutral}  & & 1.18  & 1.28  & 1.14  & 1.14  & 0.97  & 1.32  & 1.36  & 1.38  \\
\textbf{Group-01} & &  & 1.25  & 1.12  & 1.12  & 1.4   & 1.59  & 1.59  & 1.42  \\
\textbf{Group-02} & &  &  & 1.27  & 1.27  & 1.46(NS)  & 1.36  & 1.34  & 1.17  \\
\textbf{Group-03} & &  &  &  & 1.06  & 1.35(NS)  & 1.6   & 1.62  & 1.46  \\
\textbf{Group-04} & &  &  &  &  & 1.36  & 1.59  & 1.6   & 1.45  \\
\textbf{Group-05} & &  &  &  &  &  & 1.31  & 1.36  & 1.65  \\
\textbf{Group-06} & &  &  &  &  &  &  & 0.9   & 1.21  \\
\textbf{Group-07} & &  &  &  &  &  &  & & 1.16 
\end{tabular}
\caption{\textbf{Distance between prototypes for upper beta band:} The cell values in the table shows the mean distance between emotion groups' prototypes. The mean and median value calculated over all the distances mentioned in the table is 0.67 \& 0.73, respectively. NS: Not Significant
% sftp://silp150@172.17.25.150/mnt/8068a573-f543-43aa-8252-d1bf146726fa/ForMSAAnalysis/topoplotDiff.py
}
\label{tab:protodist}
\end{table}

==> SourceLocalizationRelated.tex <==
\subsection*{Source Localization}
The maps shown in the figure-\ref{FIG:AllTopoUpperBeta} are in the order of explaining the variance (the portion of EEG point topography that can be explained) in the GFP series calculated from the EEG data. The source localized representation of the particular map is calculated by taking the mean of the source localized activities on the time-stamps which were assigned an individual map. With this procedure the source localized maps for emotion conditions and baseline is created. Using non-parametric statistics, we compared these source localized maps for emotion groups with the baseline condition. We found that first map for all emotion groups generally have no/few regions of activation. And, first map is covering maximum variation in the GFP. As we move to the later source localized microstate maps, we found that later maps increasingly have more different global organization of neural activity for emotion groups than for the baseline conditions. 

Map-1 of emotional condition is not different from Map-1 of the baseline condition. That means the scalp configuration localized to brain regions for emotional and baseline condition is almost same. This result can be interpreted in two ways. First, 

Based on these results we can say that the global neuronal configuration for the baseline activity plays significant role in emotion processing. Although, there are other processes as well which are in play during emotion processing which are potentially different from the baseline processing. In other words, default mode activity is part of the whole processing related to emotional experience. 

==> Surrogate_Analysis.tex <==
https://statisticsbyjim.com/hypothesis-testing/bootstrapping/
https://towardsdatascience.com/bootstrap-and-statistical-inference-in-python-a06d098a8bfd
EEG And Microstates And Surrogate And Topography
HERMES EEG toolbox
https://www.youtube.com/watch?v=_UWRPCHBito
https://www.youtube.com/watch?v=sHnoCXj5Axs
bootstrapping with single sample
statistical inference with surrogate analysis on single sample
"surrogate analysis" of "EEG microstates"
difference between bootstrapping and surrogate analysis
surrogate analysis with EEG topography
